Contextual Bandits for Advertising Campaigns: A Diffusion-Model Independent Approach (Extended Version)

Motivated by scenarios of information diffusion and advertising in social media, we study an influence maximization problem in which little is assumed to be known about the diffusion network or about the model that determines how information may propagate. In such a highly uncertain environment, one can focus on multi-round diffusion campaigns, with the objective to maximize the number of distinct users that are influenced or activated, starting from a known base of few influential nodes. During a campaign, spread seeds are selected sequentially at consecutive rounds, and feedback is collected in the form of the activated nodes at each round. A round's impact (reward) is then quantified as the number of newly activated nodes. Overall, one must maximize the campaign's total spread, as the sum of rounds' rewards. In this setting, an explore-exploit approach could be used to learn the key underlying diffusion parameters, while running the campaign. We describe and compare two methods of contextual multi-armed bandits, with upper-confidence bounds on the remaining potential of influencers, one using a generalized linear model and the Good-Turing estimator for remaining potential (GLM-GT-UCB), and another one that directly adapts the LinUCB algorithm to our setting (LogNorm-LinUCB). We show that they outperform baseline methods using state-of-the-art ideas, on synthetic and real-world data, while at the same time exhibiting different and complementary behavior, depending on the scenarios in which they are deployed.

==> reviews_sdm.tex <==
\section{Reviews}
\subsection{Reviewer 1}

\subsubsection{1. Give a short summary of the paper, highlighting the main contributions.}
This paper presents a variation of the influence maximization problem in a more dynamic environment, with multi- round diffusion campaigns. This is in each round seeds are selected for the campaign and then the list of newly activated nodes (regarded as the reward) is collected as s feedback for subsequent campaigns. The objective is thus to maximize the total reward across all the sequence of campaigns. The paper introduces two algorithms GLM-GT- UCB and LogNorm-LinUCB based on generalized linear model and the Good-Turing estimator and the LinUCB algorithm that creates a linear combination of rewards with underlying log-normals distribution. The experiments compare these models with a few baselines on a synthetic dataset and two real world datasets (Twitter, Sina Weibo)
\subsubsection{2. List *three* main strengths of the paper.}
Identifying a sequential variation of the influence maximization problem using several interventions in a similar but different spirit than OIMP is an interesting problem of relevance to different domains where exploration and exploitation diffusion models are needed.
The proposed solutions are non-trivial in the sense that the paper does not simply propose one solution to the estimation problem but two and care was taken in the analysis of distributional assumptions at various stages such as on each influencer and context.
The estimated remaining potential is theoretically bounded and thus, performance guarantees are provided for it.
\subsubsection{3. List *three* main weaknessess of the paper}
Some decisions for the experimental evaluation require more justification. 
\red{\\For instance, why are the activation probabilities computed as a sigmoid function of the inner product of the node feature vector and the context?} \blue{Addressed\\}
The advertising campaign run on social networks that are generally highly sparse. Thus, class imbalance will affect local regions of the network which will make the feature vector (and possibly the context) asymmetric. What guarantees that enough representation is available to ensure a sigmoid is directly applicable.
\red{\\The only evaluation presented is on the cumulative rewards and no analysis is provided about the stability of the models under different parameters and hyperparameters.}\blue{NOT Addressed\\}
\red{\\Other analysis of stability that is relevant but missing from the paper is the effect of certain feature encodings in the analysis. For instance, the centroids used for the Twitter data were derived using K-means, which is highly susceptible to starting assignment of clusters, and thus sometime unstable. What was done to prevent instabilities of performance due to different initial cluster centers?}\blue{Not Addressed\\}
\subsubsection{4. Give an overall score to the paper}
In a pinch: slightly above the acceptance bar
\subsubsection{5. Give a score to the reproducibility of the experiments}
\red{Not reproducible: all the code or the data are not available, or there are no instructions}

\subsubsection{7. Write a detailed review, justifying your score and suggesting ways in which the Authors may improve the submission.}
This paper presents interesting ideas of influence maximization in a dynamic setting. I feel the methodological component of the paper is stronger than the experimental component. Thus, my evaluation and suggestions are on the later. 
\red{\\In addition to the questions I already detailed above, I suggest to include a more detailed and systematic description of the experiments. For instance, for Latent Dirichlet Allocation, what where the hyperparameters used and why.}\blue{Not done by us, reference is given}
\red{\\For K-means, what initialization policy was used for the centroid location.} \blue{random centroid initialization}
\red{\\Sampling with replacement was used for the selection of tweets by matching the context to the centroid distribution. How was this matching performed?}\blue{Addressed}
\red{\\Minor comment. There is a typo in the second paragraph of the Experiments section: "Fig. ??".}\blue{Addressed}
\subsection{Reviewer 2}

\subsubsection{1. Give a short summary of the paper, highlighting the main contributions.}
This submission tries to study contextual bandits for advertising campaigns with a diffusion-model independent approach to maximize the rewards or influence, and tested on Twitter and Weibo data sets.
\subsubsection{2. List *three* main strengths of the paper.}
1. this draft is easy to follow
2. your centroids are obtained via clustering 3. two real-world data are employed
\subsubsection{3. List *three* main weaknessess of the paper}
\red{\\1. your main baselines are weak, there are related state-of-the-art you are encouraged to compare: Distributed Clustering of Linear Bandits in Peer to Peer Networks, Fast Distributed Bandits for Online Recommendation Systems, Collaborative Filtering Bandits}\blue{Not Addressed}
\red{\\2. the scale of your experiments is a bit small, to make it more comprehensive try to import new real-world and larger scale data, and enlarge the number of rounds, especially in nowadays distributed big data scenarios} \blue{Not Addressed}
\red{\\3. spend an effort to tune your regret analysis and try to unify it with consistent experimental performance} \blue{Unclear}
\subsubsection{4. Give an overall score to the paper}
Should accept: in the 80\% best papers of SDM
\subsubsection{5. Give a score to the reproducibility of the experiments}
Clearly reproducible: code and data are available, and there are instructions for how to reproduce it
\subsubsection{7. Write a detailed review, justifying your score and suggesting ways in which the Authors may improve the submission.}
It's enjoyable to have a read for this submission, however, there are some jobs that need to be done to better improve it, especially like q3, overall, I found it has made some reasonable attempts and have no problem to give a chance for this interesting draft.
\subsection{Reviewer 3}

\subsubsection{1. Give a short summary of the paper, highlighting the main contributions.}
This paper studies the problem of online influence maximization, under the condition that diffusion network topologies, the influence probabilities, and the underlying diffusion model are unknown. Instead, the potential spread initiators are offered as prior knowledge. To address this problem, the authors modified an existing contextual multi-armed bandits framework to model the original problem, with the assumption that contextual information is known and exploitable in the sequential learning process. Combining this contextual multi-armed bandits framework with two distinct assumption on the underlying distributions of the number of influenced nodes, the authors proposed two UCB-like algorithms as well as the corresponding theoretical regret analysis. Experiments on both real and synthetic datasets show the efficiency and effectiveness of the proposed method.
\subsubsection{2. List *three* main strengths of the paper.}
(1) The authors address the problem of online influence maximization, which is an interesting problem and relevant to a wide community of researchers.
(2) Experiments were conducted on both real and synthetic datasets show the efficiency and effectiveness of the proposed method.
(3) Theoretical analysis are provided to guarantee the validity of proposed method.
\subsubsection{3. List *three* main weaknessess of the paper}
(1) There are some explicit assumptions, which is probably inconsistent with the reality scenario. 
\red{\\(2) The strategy of choosing the influencers to be updated is limited.}\blue{Not Addressed}
(3) The discussion of the experimental evaluation and the results is marginally inadequate.
\subsubsection{4. Give an overall score to the paper}
In a pinch: slightly above the acceptance bar
\subsubsection{5. Give a score to the reproducibility of the experiments}
Almost reproducible: either some minor parts of the code or some data is not available, or some of the instructions are unclear
\subsubsection{7. Write a detailed review, justifying your score and suggesting ways in which the Authors may improve the submission.}
The problem addressed in the paper (online influence maximization) is relevant and framing this problem within contextual multi-armed bandits setting is interesting. I do, however, have some concerns about the paper, which I have tried to detail below:
\red{\\a. Assumptions: The authors make assumptions on the underlying distributions of the number of influenced nodes, i.e., Poisson distribution and log-normal distribution. Can those distributions simulate the reality situation? Is there any basis?}
\red{\\b. Choosing influencers to be updated: In this paper, the authors propose to choose L influencers with the largest UCB. For this, what if the remaining potential of these influencers overlap with each other? Maybe it is better to choose the influencers to be updated in a combinatorial pattern, taking the overlap into consideration?\\}
c. Experimental evaluation:
\red{\\(1) According to the paper, the proposed method is model-independent. However, in synthetic data experiments, the authors only utilized IC model to generate the synthetic diffusion data. Only testing the algorithms with IC model is insufficient to verify the “model-independent” property of the algorithm.}
\red{\\(2) As for the baselines, UCB1 [4] and LinUCB [10] seem to be outdated. Besides, both of them are general frameworks for Bandit-based problems, rather than approaches specifically targeting at IM problem. So, I really do not think they are the appropriate choices to be compared. Maybe [27, 28, 29] are better.}
\red{\\(3) The experimental results did not testify to the robustness of the proposed algorithms. It is better to test the algorithm with more different experimental settings, like different diffusion network size (number of nodes K), regulation factor $\gamma$, number of selections L, etc.}
d. Typos:
In page 7. “Fig. ?? of the supplementary”
\red{\\In page 9. “both theoretically and experimentally than” ->“both theoretically and experimentally that”}\blue{Fixed}

\subsection{Reviewer 4}

\subsubsection{1. Give a short summary of the paper, highlighting the main contributions.}
This paper studies the online influence maximization in which the influencers are formulated as arms and the newly activated nodes are regarded as rewards. To balance the exploitation and exploration dilemma in this scenario, the authors propose UCB-based bandit algorithms, and the theoretical and empirical evaluation are provided.
\subsubsection{2. List *three* main strengths of the paper.}
1. This is an elaborate paper, where the motivation is clear and the design of the algorithm is built on reasonable intuition and theoretical analysis.
2. The authors propose a good-tuning estimator coming with fatigue, which enables the regret definition to be more rigorous.
3, The two proposed algorithms consider different assumptions on rewards, e.g., Poison and Log-normal, which extend the coverage of reward formulation.
\subsubsection{3. List *three* main weaknessess of the paper}
1. The experiment part can be improved, where more recent SOTA baselines can be put in comparison. 2. The figure in page 7 is missing.
\subsubsection{4. Give an overall score to the paper}
In a pinch: slightly above the acceptance bar
\subsubsection{5. Give a score to the reproducibility of the experiments}
Almost reprodicible: either some minor parts of the code or some data is not available, or some of the instructions are unclear
\subsubsection{7. Write a detailed review, justifying your score and suggesting ways in which the Authors may improve the submission.}
In general, I like this paper which proposes a new estimator for potential of influencer embedded in UCB-based bandit algorithms, and the presentation is good, except that the experiments can be further improved.
\subsection{Reviewer 5}
Questions
\subsubsection{1. Give a short summary of the paper, highlighting the main contributions.}
This paper studies the problem of influence maximization when neither the graph topology nor the activation model is known a priori. To balance between exploration and exploitation, the authors proposed to solve the problem using multi-armed bandits. Compared with the existing literature pursuing this direction, the key differentiator of this paper is the introduction of contextual information, which allows a more nuanced activation model that takes into account the potential variation of messages propagated in different rounds.
\subsubsection{2. List *three* main strengths of the paper.}
S1. The paper was very clearly written and a joy to read.
S2. The authors presented a thoughtful technical treatment of the problem.
\subsubsection{3. List *three* main weaknessess of the paper}
\red{\\W1. It is not quite clear how GLM-GT-UCB and LogNorm-LinUCB complement each other in real-world settings.}
\red{\\W2. It would be helpful to provide some empirical evidence demonstrating the importance of contextual information in real-world influence maximization campaigns.}
\subsubsection{4. Give an overall score to the paper}
In a pinch: slightly above the acceptance bar
\subsubsection{5. Give a score to the reproducibility of the experiments}
Clearly reproducible: code and data are available, and there are instructions for how to reproduce it
\subsubsection{7. Write a detailed review, justifying your score and suggesting ways in which the Authors may improve the submission.}
This paper contributes to the literature of using multi-armed bandits algorithms to solve influence maximization problems over social networks. The key novelty of this paper is the introduction of contextual information, which allows information known about the context to be exploited in the learning process. To handle the context information, the authors developed two algorithms, one based on the Good Turing estimator and the other based on the LinUCB algorithm. The paper includes a set of theoretical and experimental results that demonstrate the effectiveness of the algorithms.
Overall, this is a nicely written paper that presents a piece of well executed work. I think it nicely complements the emerging literature on using multi-armed bandits for influence maximization. Nonetheless, I also have two concerns, one technical and one practical. 
\red{The technical concern is that the LinUCB-based algorithm appears to perform rather well on all real-world datasets tested in the paper. This begs the question of whether (and when) the algorithm based on Good Turing estimator is useful in practice. The authors stated in the introduction that the two algorithms complement each other. Some elaborations on this point would be appreciated.}\blue{Not Fixed}
\red{\\The other concern I have is on the practical impact of the work. While the experimental results demonstrate the power of the algorithms, the importance of the contextual information is essentially determined by the experimental settings. As such, some empirical evidence on the power of contextual information in practice would be appreciated.}


